Model-Free Opponent Shaping

In general-sum games, the interaction of self-interested learning agents commonly leads to collectively worst-case outcomes, such as defect-defect in the iterated prisoner's dilemma (IPD). To overcome this, some methods, such as Learning with Opponent-Learning Awareness (LOLA), shape their opponents' learning process. However, these methods are myopic since only a small number of steps can be anticipated, are asymmetric since they treat other agents as naive learners, and require the use of higher-order derivatives, which are calculated through white-box access to an opponent's differentiable learning algorithm. To address these issues, we propose Model-Free Opponent Shaping (M-FOS). M-FOS learns in a meta-game in which each meta-step is an episode of the underlying inner game. The meta-state consists of the inner policies, and the meta-policy produces a new inner policy to be used in the next episode. M-FOS then uses generic model-free optimisation methods to learn meta-policies that accomplish long-horizon opponent shaping. Empirically, M-FOS near-optimally exploits naive learners and other, more sophisticated algorithms from the literature. For example, to the best of our knowledge, it is the first method to learn the well-known Zero-Determinant (ZD) extortion strategy in the IPD. In the same settings, M-FOS leads to socially optimal outcomes under meta-self-play. Finally, we show that M-FOS can be scaled to high-dimensional settings.

==> outline.tex <==
1. Abstract (DO LAST)

2. Introduction
    1. Talk about MARL and Competitive vs. Cooperative vs. General-Sum and why General-Sum is relevant.
    % 2. Talk about Meta-Learning (?)
    2. Talk about the IPD as an example and why existing algorithms fail to perform well.
    3. Talk about LOLA
        a. Gets TFT in IPD
        b. Assumes opponent is a naive learner
    4. Talk about shortcomings of LOLA
        a. Myopic
        b. Second-Order Derivatives
        c. Inconsistent
        d. Assumes opponent learning model (does not work against arbitrary opponents)
    5. Introduce M-FOS and brief description of how it works. 
        a. Meta-Learning algorithm across multiple learning episodes of the opponent.
        b. Makes no assumptions about the opponent's learning model.
        c. Considers the opponent's policy throughout an infinite episode (not myopic).
    6. M-FOS Results:
        a. M-FOS performs better than baseline algorithms against all opponents in H2H Table in a variety of games. This includes LOLA. M-FOS is the first algorithm that learns to exploit LOLA.
        b. Against Naive Learners, in the IPD, M-FOS discovers a strategy called Extortion. This is first learning algroithm to do this.
        c. Against itself, M-FOS learns to cooperate in the IPD. We also believe that this is the first method that does not use higher-order gradients to achieve cooperation in the IPD.
        d. We demonstrate that M-FOS can scale to a more complex temporally-extended social dilemmas.

3. Related Work
    1. CHRIS WILL DO THIS STUFF 
    2. Compare and Contrast
    3. Kim et al. cheat, they meta-learn initialization parameters and hardcode the update whereas we start with random parameters and meta-learn the update function. They also assume that opponent is a naive policy gradient learning agent.
    
4. Background
    1. Notation.
        a. Differentiable Games. Introduce exact value function, access to opponent parameters, and differentiability of environment. 
    2. Naive Learning
        a. Introduce vbasic gradient ascnet.
    3. LOLA
        a. Introduce LOLA. Don't introduce LOLA-PG cuz it doesnt work.
    4. SOS and other methods
    5. Meta-Learning
    
5. Method Section
    1. Algorithm description
        a. General Meta-Learning Setup. Talk about learning across multiple inner episodes of the opponent. 
        b. M-FOS applied on simple games. 
        c. M-FOS applied on sequential games
    2. Hyperparameters
    3. Update function
    5. Paragraph about how M-FOS is a general meta-learning algorithm and we demonstrate it on the Coin game
    5. Pseudocode (see Kim et al.)

    
6. Experimental Setup
    1. We compare against a set of other general-sum learning methods (LOLA, SOS and NL)
    2. We compare against a static opponent
    3. Comparison (or lack thereof) with Kim et al. Can we extort Kim et al?
    
Appendix
    1. Pseudo Code for Coin Game
    
    
    https://arxiv.org/abs/2102.09381
    https://arxiv.org/abs/2011.00382
    https://arxiv.org/abs/2108.01843
    https://arxiv.org/abs/2006.06051
    https://arxiv.org/abs/2011.06619
    https://arxiv.org/abs/1707.06347
    https://github.com/nikhilbarhate99/PPO-PyTorch
    https://arxiv.org/abs/1712.06567
    https://arxiv.org/abs/1703.03864
    https://arxiv.org/abs/1803.07055
    
    https://arxiv.org/abs/1611.02779
    https://arxiv.org/abs/1703.03400
    https://arxiv.org/abs/2201.04182
    
    
    FIGURES:
    1. M-FOS PSEUDO CODE.
        A. INCLUDE PARTS / DEFINITIONS THAT YOU SWAP OUT FOR THE TWO DIFFERENT IMPLEMENTATIONS
    2. M-FOS IPD TABLE RESULTS (DONE?)
    3. M-FOS IMP TABLE RESULTS (DONE?)
    4. M-FOS TANDEM TABLE RESULTS (DONE?)
    5. M-FOS v. NL IPD POLICY PLOT ()
    % 5.5. M-FOS v. LABR IPD POLICY PLOT?
    6. M-FOS v. LOLA IPD POLICY PLOT
    7. M-FOS v. M-FOS IPD POLICY PLOT
    
    (DEMONSTRATES NON-MYOPIC)
    8. M-FOS v. NL IMP POLICY PLOT (?)
    9. LOLA v. NL IMP POLICY PLOT (?)
    
    10. COIN GAME TRAINING PLOTS FOR DIFFERENT LAMBDAS
    11. COIN GAME \% OWN PICKED UP TRAINING PLOT FOR DIFFERENT LAMBDAS
    12. 
    
    
    
    
